GeoNet: Benchmarking Unsupervised Adaptation across Geographies

In recent years, several efforts have been aimed at improving the robustness of vision models to domains and environments unseen during training. An important practical problem pertains to models deployed in a new geography that is under-represented in the training dataset, posing a direct challenge to fair and inclusive computer vision. In this paper, we study the problem of geographic robustness and make three main contributions. First, we introduce a large-scale dataset GeoNet for geographic adaptation containing benchmarks across diverse tasks like scene recognition (GeoPlaces), image classification (GeoImNet) and universal adaptation (GeoUniDA). Second, we investigate the nature of distribution shifts typical to the problem of geographic adaptation and hypothesize that the major source of domain shifts arise from significant variations in scene context (context shift), object design (design shift) and label distribution (prior shift) across geographies. Third, we conduct an extensive evaluation of several state-of-the-art unsupervised domain adaptation algorithms and architectures on GeoNet, showing that they do not suffice for geographical adaptation, and that large-scale pre-training using large vision models also does not lead to geographic robustness. Our dataset is publicly available at https://tarun005.github.io/GeoNet.

==> tables/Rebuttal_Tables/NoiseAccuracy.tex <==
\begin{table}[!t]
  \centering
  \resizebox{0.35\textwidth}{!}{
  % \begin{tabular}{@{} >{\raggedright}p{5.2cm} >{\raggedright}p{2.2cm} >{\raggedright}p{2.2cm} >{\raggedright}p{2cm} p{2cm}}
  \begin{tabular}{lccccccccc}
    Noise (\%) $\rightarrow$ & 0\% & 1\% & 5\% & 10\% & 20\% & 50\% \\
    \cline{2-7}
    & \multicolumn{6}{c}{\textbf{\underline{\GeoP}}}  \\
    USA   & 55.9 & 55.9 & 55.2 & 55.0 & 53.6 & 48.6 \\
    Asia  & 37.0 & 36.9 & 36.6 & 35.8 & 35.5 & 32.3  \\
    $\Delta(\%)$ & \textcolor{brown}{18.9} & \textcolor{brown}{19.0} & \textcolor{brown}{18.6} & \textcolor{brown}{19.2} & \textcolor{brown}{18.1} & \textcolor{brown}{16.3} \\
    \cline{2-7}
    & \multicolumn{6}{c}{\textbf{\underline{\GeoI}}}  \\
    USA   & 46.6 & 46.5 & 45.8 & 44.7 & 43.7 & 36.9  \\
    Asia  & 29.5 & 29.5 & 29.2 & 28.5 & 27.9 & 23.1 \\
    $\Delta(\%)$ & \textcolor{brown}{17.1} & \textcolor{brown}{17.0} & \textcolor{brown}{16.6} & \textcolor{brown}{16.2} & \textcolor{brown}{15.8} & \textcolor{brown}{13.8} \\
    \bottomrule
  \end{tabular}
  }
  \vspace{-1em}
  \captionsetup{width=0.45\textwidth}
  \caption{\label{tab:noise-acc} USA ${\rightarrow}$ Asia transfer across geographies with varying label noise. }
  \vspace{-16pt}
\end{table}

==> tables/Rebuttal_Tables/RandomMix.tex <==
\begin{table}[!t]
  \centering
  \resizebox{0.36\textwidth}{!}{
  % \begin{tabular}{@{} >{\raggedright}p{5.2cm} >{\raggedright}p{2.2cm} >{\raggedright}p{2.2cm} >{\raggedright}p{2cm} p{2cm}}
  \begin{tabular}{lccccccccc}
    \% of Asia Data & 0\% & 50\% & 100\% \\
    % \cline{2-4} \cline{6-8}
    USA Acc. &  55.6 & 51.9 & 21.2 \\
    Asia Acc. & 36.3 & 49.5 & 50.6 \\
    Drop (\%) & 19.3\% & 2.4\% & 29.4\% \\
    \bottomrule
  \end{tabular}
  }
  \vspace{-1em}
  \captionsetup{width=0.45\textwidth}
  \caption{\label{tab:random-mix} Cross-geography transfer with domain-mixed datasets.}
  \vspace{-1em}
\end{table}

==> tables/dataset_overview.tex <==
\begin{table*}[!t]
  \centering
  \resizebox{0.75\textwidth}{!}{
  % \begin{tabular}{@{} >{\raggedright}p{5.2cm} >{\raggedright}p{2.2cm} >{\raggedright}p{2.2cm} >{\raggedright}p{2cm} p{2cm}}
  \begin{tabular}{lccccc}
    \toprule  \\[-1em]
    Dataset & \#Images & \#Classes & Category Type & Shift Type & Metadata \\
    \midrule
    Office-31~\cite{office31} & 4.1k & 31 & Objects & Web/real/dslr & \cross \\
    Office-Home~\cite{venkateswara2017deep} & 15.5k & 65 & Objects & Style & \cross \\
    visDA~\cite{peng2017visda} & 207k & 12 & Objects & sim2real & \cross \\
    DomainNet~\cite{peng2019moment} & 587k & 345 & Objects & style & \cross \\
    Dollar Street~\cite{DBLP:journals/corr/abs-1906-02659, prabhu2022can} & 11.7k & 58 & Objects & Household income & \cross \\
    \midrule
    \textit{Proposed Benchmark} \\
    \GeoI & - & - & Objects & \multirow{2}{*}{Geographies} & \multirow{2}{*}{\tick}  \\
    % \multirow{2}{*}{GPS coordinates, hashtags, textual captions}
    \GeoP & 567k & 205 & Places/Scenes \\
    \bottomrule \\
  \end{tabular}
  }
  \vspace{-1em}
  \captionsetup{width=0.9\textwidth}
  \caption{\label{tab:comparison-table} Comparison of existing benchmarks for unsupervised domain adaptation. In contrast to existing benchmarks, \Ours{} is the first large-scale benchmark to study the problem of geographical domain adaptation across diverse tasks like scene and object classification,  }
  \vspace{-1em}
\end{table*}

==> tables/src_transfer_and_UDA_table_And_fig.tex <==
\begin{table*}[!t]
    \begin{minipage}[b]{.45\linewidth}
    %
        \begin{minipage}{\linewidth}
            \centering
              \resizebox{\textwidth}{!}{
              % \begin{tabular}{@{} >{\raggedright}p{5.2cm} >{\raggedright}p{2.2cm} >{\raggedright}p{2.2cm} >{\raggedright}p{2cm} p{2cm}}
              \begin{tabular}{lccccccccc}
                & \multicolumn{3}{c}{\textbf{\underline{\GeoP}}}  \\
                Train $\downarrow$ / Test $\rightarrow$ & USA & Asia & Drop (\%) \\
                \cline{2-4}
                USA & 55.60/84.89 & 36.29/64.29 & \textcolor{brown}{-19.31/-20.60} \\
                Asia & 21.20/45.57 & 50.60/78.82 & \textcolor{brown}{-29.40/-33.25} \\
                % \textcolor{gray}{USA+Asia} & \textcolor{gray}{yy.yy/yy.yy} & xx.xx/xx.xx &  \\
                \midrule 
                & \multicolumn{3}{c}{\textbf{\underline{\GeoI}}} \\
                Train $\downarrow$ / Test $\rightarrow$ & USA & Asia & Drop (\%) \\
                \cline{2-4}
                USA & 46.63/67.85 & 29.69/51.43 & \textcolor{brown}{-16.94/-16.42} \\
                Asia & 31.55/52.28 & 52.93/72.96 & \textcolor{brown}{-21.38/-20.68} \\
                % \textcolor{gray}{USA+Asia} & \textcolor{gray}{yy.yy/yy.yy} & \textcolor{gray}{xx.xx/xx.xx} &  \\
                \bottomrule
              \end{tabular}
              }
              \vspace{-1em}
              \captionsetup{width=\textwidth}
              \subcaption{\label{tab:source-transfer}}
              \vspace{-1em}
        \end{minipage}

        \begin{minipage}{\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/GeoImnet-groups.pdf}
            \subcaption{\label{fig:imnet-groupdrops}
            }
            \vspace{-16pt}
        \end{minipage}
    \end{minipage}
    \hfill
    \begin{minipage}[b]{.5\linewidth}
        \centering
          % \rowcolors{2}{gray!25}{white}
          \resizebox{\textwidth}{!}{
          % \begin{tabular}{@{} >{\raggedright}p{5.2cm} >{\raggedright}p{2.2cm} >{\raggedright}p{2.2cm} >{\raggedright}p{2cm} p{2cm}}
          \begin{tabular}{lccccccccccc}
          \toprule
            Method & \multicolumn{4}{c}{\underline{\GeoP}} && \multicolumn{4}{c}{\underline{\GeoI}}  \\
            % \cline{2-12}
                     & \multicolumn{2}{c}{USA $\rightarrow$ Asia} & \multicolumn{2}{c}{Asia $\rightarrow$ USA} && \multicolumn{2}{c}{USA $\rightarrow$ Asia} & \multicolumn{2}{c}{Asia $\rightarrow$ USA} \\
                     \midrule
                                            & Top-1 & Top-5 & Top-1 & Top-5 && Top-1 & Top-5 & Top-1 & Top-5 \\
                                            \cline{2-5} \cline{7-10}
            % \midrule
             Source Only                    & \textbf{37.10} & \textbf{64.08} & \textbf{21.19} & \textbf{45.57} && \underline{29.69} & \underline{51.43} & \textbf{31.55} & \textbf{52.28} \\
             DANN~\cite{DANN}               & 30.42 & 56.33 & 16.68 & 35.90 && 27.15 & 48.06 & 30.17 & 50.48 \\
             CDAN~\cite{CDAN}               & 30.58 & 56.68 & 17.11 & 36.10 && 28.22 & 49.09 & 30.72 & 51.44 \\
             MCC~\cite{jin2020minimum}      & 30.78 & 56.83 & 17.88 & 37.32 && 28.55 & 49.50 & 30.86 & 51.52 \\
             SAFN~\cite{xu2019larger}       & 31.38 & 57.57 & 14.77 & 36.30 && 23.23 & 45.53 & 28.53 & 49.23 \\
             MDD~\cite{zhang2019bridging}   & \underline{32.28} & \underline{59.55} & 14.23 & 34.34 && \textbf{29.75} & \textbf{51.90} & \underline{31.17} & 51.51 \\
             MCD~\cite{saito2018maximum}    & 31.62 & 59.16 & 16.03 & 33.75 && 24.22 & 44.51 & 27.53 & 48.36 \\
             ToAlign~\cite{wei2021toalign}  & 29.70 & 57.32 & 16.74 & 35.54 && 26.65 & 47.73 & 28.55 & 50.10 \\
             MemSAC~\cite{kalluri2022memsac}& 31.64 & 57.69 & \underline{18.41} & \underline{38.34} && 28.73 & 50.65 & 31.04 & \underline{52.11} \\ 
             \midrule
             \textcolor{lightgray}{Tgt. Supervised} & \textcolor{lightgray}{50.60} & \textcolor{lightgray}{78.82} &\textcolor{lightgray}{55.60} & \textcolor{lightgray}{84.89} && \textcolor{lightgray}{52.93} & \textcolor{lightgray}{72.96} & \textcolor{lightgray}{46.63} & \textcolor{lightgray}{67.85} \\
            \bottomrule
          \end{tabular}
          }
          \vspace{-1em}
          \captionsetup{width=0.45\textwidth}
          \caption{\label{tab:uda-benchmarking}}
          \vspace{-1em}
    \end{minipage}
\end{table*}

==> tables/src_transfer_and_figure.tex <==
\begin{table*}[!t]
    \begin{minipage}[b]{0.48\linewidth}
        \centering
          \resizebox{\textwidth}{!}{
          % \begin{tabular}{@{} >{\raggedright}p{5.2cm} >{\raggedright}p{2.2cm} >{\raggedright}p{2.2cm} >{\raggedright}p{2cm} p{2cm}}
          \begin{tabular}{lccccccccc}
            & \multicolumn{3}{c}{\textbf{\underline{\GeoP}}}  \\
            Train $\downarrow$ / Test $\rightarrow$ & USA & Asia & Drop (\%) \\
            \cline{2-4}
            USA & 55.60/84.89 & 36.29/64.29 & \textcolor{brown}{-19.31/-20.60} \\
            Asia & 21.20/45.57 & 50.60/78.82 & \textcolor{brown}{-29.40/-33.25} \\
            % \textcolor{gray}{USA+Asia} & \textcolor{gray}{yy.yy/yy.yy} & xx.xx/xx.xx &  \\
            \midrule 
            & \multicolumn{3}{c}{\textbf{\underline{\GeoI}}} \\
            Train $\downarrow$ / Test $\rightarrow$ & USA & Asia & Drop (\%) \\
            \cline{2-4}
            USA & 46.63/67.85 & 29.69/51.43 & \textcolor{brown}{-16.94/-16.42} \\
            Asia & 31.55/52.28 & 52.93/72.96 & \textcolor{brown}{-21.38/-20.68} \\
            % \textcolor{gray}{USA+Asia} & \textcolor{gray}{yy.yy/yy.yy} & \textcolor{gray}{xx.xx/xx.xx} &  \\
            \bottomrule
          \end{tabular}
          }
          \captionsetup{width=\textwidth}
          \subcaption{\label{tab:source-transfer}}
          \vspace{-16pt}
    \end{minipage}
    ~~
    \begin{minipage}[b]{0.48\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/GeoImnet-groups.pdf}
        \subcaption{\label{fig:imnet-groupdrops}
        }
        \vspace{-16pt}
    \end{minipage}
    \caption{}
\end{table*}

==> tables/unida_and_vit.tex <==
\begin{table*}[!t]
    \begin{minipage}[t]{0.45\linewidth}
        \centering
          \resizebox{\textwidth}{!}{
          % \begin{tabular}{@{} >{\raggedright}p{5.2cm} >{\raggedright}p{2.2cm} >{\raggedright}p{2.2cm} >{\raggedright}p{2cm} p{2cm}}
          \begin{tabular}{lccccc}
            Method & Closed-set acc. & Open-set acc. & H-Score && Tgt Sup.  \\
            \midrule
            UniDA~\cite{you2019universal} & 27.64 & 43.93 & 33.93 && \multirow{3}{*}{\textcolor{gray}{70.70\%}}  \\
            DANCE~\cite{saito2020dance} & 38.54 & 78.73 & 51.75 &&  \\
            OVANet~\cite{saito2021ovanet} & 36.54 & 66.89 & 47.26 &&  \\
            \bottomrule
              \end{tabular}
              }
          \vspace{-1em}
          \captionsetup{width=0\textwidth}
          \caption{\label{tab:uniDA-benchmarking} {\bf Accuracy of universal domain adaptation methods on the proposed Geo-UniDA benchmark}. \textit{Closed} refers to the closed set accuracy on the shared classes, \textit{open} refers to the OOD detection accuracy and \textit{H-Score} is the average of the two.}
          \vspace{-1em}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.45\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/ViT-places.pdf}
        \caption{{\bf USA $\rightarrow$ Asia on \GeoP{}}.
        }
        \label{fig:vit-places}
        \vspace{-10pt}
    \end{minipage}
\end{table*}

==> tables/vit_benchmarks.tex <==
\begin{table*}[!t]
  \centering
  % \rowcolors{2}{gray!25}{white}
  \resizebox{0.8\textwidth}{!}{
  % \begin{tabular}{@{} >{\raggedright}p{5.2cm} >{\raggedright}p{2.2cm} >{\raggedright}p{2.2cm} >{\raggedright}p{2cm} p{2cm}}
  \begin{tabular}{lccccccccccc}
  \toprule
    Backbone & \multicolumn{2}{c}{{Pre-Training}} & \multicolumn{4}{c}{\GeoP} & \multicolumn{4}{c}{\GeoI}  \\
    % \cline{2-12}
             & Data & Method & \multicolumn{2}{c}{USA $\rightarrow$ Asia} & \multicolumn{2}{c}{Asia $\rightarrow$ USA} & \multicolumn{2}{c}{USA $\rightarrow$ Asia} & \multicolumn{2}{c}{Asia $\rightarrow$ USA} \\
    
    \midrule
             &&& Top-1 & Top-5 & Top-1 & Top-5 & Top-1 & Top-5 & Top-1 & Top-5 \\
    % \cline{5-6} \cline{7-8} \cline{9-10} \cline{11-12} 
    %% Resnet
    \multirow{4}{*}{\begin{tabular}{@{}c@{}}Resnet-50 \\ (23.5M)\end{tabular}} %
                               & IN1k & Sup.& 37.10 & 64.08 & 19.24 & 42.02 & 28.28 & 48.64 & 28.37 & 48.52 \\
                               & IN1k & MoCo & 36.97 & 64.31 & 20.14 & 42.74 & 26.12 & 46.7 & 25.82 & 46.01 \\
                               & IN1k & SWAV & 38.29 & 64.82 & 17.87 & 37.99 & 26.89 & 47.96 & 28.5 & 49.11 \\
                               & IN1k & DINO & 37.66 & 63.69 & 17.45 & 37.13 & 26.55 & 47.75 & 28.23 & 48.98 \\
    & \multicolumn{2}{c}{\textcolor{gray}{Tgt. Supervised}} & \\
    \midrule
    \multirow{2}{*}{\begin{tabular}{@{}c@{}}ViT-small \\ (22.5M)\end{tabular}} %
                               & IN1k & Sup. & 40.7 & 68.16 & 26.78 & 53.71 & 31.56 & 52.7 & 33.9 & 54.3 \\
                               & IN1k & DINO & 37.86 & 64.29 & 20.57 & 43.78 & 26.64 & 47.49 & 26.46 & 46.21 \\
    & \multicolumn{2}{c}{\textcolor{gray}{Tgt. Supervised}} & \\
    \midrule
    \multirow{4}{*}{\begin{tabular}{@{}c@{}}ViT-base \\ (85.9M)\end{tabular}}  %
                               & IN1k & Sup. & 42.07 & 69.43 & 28.25 & 55.04 & 34.14 & 55.15 & 35.98 & 56.09 \\
                               & IN1k & DINO & 41.97 & 68.9 & 22.25 & 44.79 & 30.66 & 52.47 & 31.93 & 52.79 \\
                               & IN1k & MAE  & 37.78 & 65.01 & 17.31 & 36.53 & 25.21 & 47.0 & 27.3 & 48.7 \\
                               & IG 3.7B & SWAG & 44.962 & 70.976 & 29.27 & 53.46 & 37.56 & 60.04 & 36.56 & 57.26 \\
    & \multicolumn{2}{c}{\textcolor{gray}{Tgt. Supervised}} & \\
    \midrule
    \multirow{4}{*}{\begin{tabular}{@{}c@{}}ViT-large \\ (303.3M)\end{tabular}}  %
                               & IN21k+IN1k & Sup. & 50.14 & 75.03 & 30.96 & 55.69 & 47.29 & 65.43 & 45.96 & 64.58 \\
                               & IN1k & MAE  & 42.78 & 69.38 & 21.06 & 43.05 & 31.78 & 54.26 & 33.28 & 54.58 \\
                               & IG 3.7B & SWAG & 48.49 & 73.32 & 32.76 & 56.87 & 43.31 & 63.86 & 41.03 & 61.52 \\
    & \multicolumn{2}{c}{\textcolor{gray}{Tgt. Supervised}} & \\
    \bottomrule
  \end{tabular}
  }
  \vspace{-1em}
  \captionsetup{width=0.96\textwidth}
  \caption{\label{tab:source-transfer} Drop in accuracies caused by transfer of models across geographically different train and test domains. Note the significant drop in accuracies caused by the geographical domain shift in each setting.}
  \vspace{-1em}
\end{table*}
